Conformance Checking Based on Multi-Perspective Declarative Process Models

Process mining is a family of techniques that aim at analyzing business process execution data recorded in event logs. Conformance checking is a branch of this discipline embracing approaches for verifying whether the behavior of a process, as recorded in a log, is in line with some expected behaviors provided in the form of a process model. The majority of these approaches require the input process model to be procedural (e.g., a Petri net). However, in turbulent environments, characterized by high variability, the process behavior is less stable and predictable. In these environments, procedural process models are less suitable to describe a business process. Declarative specifications, working in an open world assumption, allow the modeler to express several possible execution paths as a compact set of constraints. Any process execution that does not contradict these constraints is allowed. One of the open challenges in the context of conformance checking with declarative models is the capability of supporting multi-perspective specifications. In this paper, we close this gap by providing a framework for conformance checking based on MP-Declare, a multi-perspective version of the declarative process modeling language Declare. The approach has been implemented in the process mining tool ProM and has been experimented in three real life case studies.

==> sections/algorithms-old.tex <==
\section{Conformance Checking Algorithms}
\label{sec:algorithms}

In this section, we describe the proposed algorithms for the conformance checking of \MPDeclare~ constraints. Each of them can be used to check the conformance of a log with respect to constraints referring to different \MPDeclare~ templates. Then, every algorithm takes as input a log and a reference \MPDeclare~ constraint. The algorithms produce as output two sets containing the positions in the log corresponding to fulfillments and violations for that constraint in each trace of the log.


%the percentage of traces in the log in which each candidate constraint is non-vacuously satisfied (the support of the candidate constraint in the log) and a vector containing the time distances between each activation and the corresponding target. The support value is used to filter out candidate constraints that are non-vacuously satisfied in a low percentage of log traces (with respect to a user-defined threshold).
%The time distances are used to
%derive statistics on the delays between activations and targets of the candidate constraint. In particular, they are used to
%identify the time interval $[t_1,t_2]$ characterizing the discovered metric temporal constraint (see Section~\ref{sec:interval}).

In the following sections, we describe the algorithms we use for the conformance checking of positive relation constraints. The same algorithms can be used also for the conformance checking of negative relation constraints taking into account that fulfillments for positive relation constraints are violations for negative relation constraints and vice versa.



\subsection{Multi-Perspective Response, Precedence, and Responded Existence constraints}
\label{response}

The algorithm presented in this section (Algorithm~\ref{alg:response}) can be used for
\emph{response} constraints.
%We illustrate the algorithm (Algorithm~\ref{alg:response})
%for the response template. The algorithm is identical for the not response
%template, since the fulfillment ratio for a response constraint corresponds to
%the violation ratio of the not response constraint over the same activities (and
%vice versa).\footnote{A similar observation also applies to the algorithms described in the following sections.}
A similar algorithm (with small modifications) is able to discover \emph{precedence} and \emph{responded existence} constraints.


The inputs of this algorithm are an event log $log$ and a multi-perspective constraint with activation $a$, target $t$, activation condition $\varphi_a$, correlation condition $\varphi_c$, and time condition $\varphi_t$. The outputs of the algorithm are two arrays of lists $\textit{fulfillments}$ and $\textit{violations}$ (one of each for each trace) containing the fulfillments and the violations in each trace with respect to the given constraint.

For each trace $trace$ in $log$, $\textit{fulfillments}_{trace}$ and $\textit{violations}_{trace}$ contain the fulfillments and the violations in trace $trace$ with respect to the reference constraint. $\textit{pendingActivations}_{trace}$ is a vector containing the pending activations in $trace$ for the reference constraint, i.e., the activations that do not have a corresponding target.

For each event $event$ in $trace$, $event$ is a pending activation if its event name is equal to $a$ and condition $\varphi_a$ is satisfied on the payload of $event$ ($event$ is an activation and is not associated to any target yet). The activation condition is evaluated through function $check_a$ (line 5). In this case, $event$ is added to $\textit{pendingActivations}_{trace}$ (lines 6). On the other hand, if the event name of $event$ is equal to $t$, $event$ is a possible target corresponding to one of the pending activations in $\textit{pendingActivations}_{trace}$. In this case, if a pending activation $p$ in $\textit{pendingActivations}_{trace}$ can be correlated to $event$ through the correlation condition $\varphi_c$ and the time condition $\varphi_t$ (the algorithm checks if this is the case through functions $check_c$ and $check_t$), then $p$ is removed from the set of pending activations and is added to $\textit{fulfillments}_{trace}$ (lines 10 and 11). When all the events in $trace$ have been processed, all the activations that are still in $\textit{pendingActivations}_{trace}$ are moved to $\textit{violations}_{trace}$ (lines 13 and 14).

%The candidate constraint under examination is non-vacuously satisfied in $trace$, if, when all the events in $trace$ have been processed, the boolean variable $activated$ is true ($trace$ contains at least one activation of the candidate constraint) and all the activations in $trace$ have a corresponding target (i.e., if $\textit{pendingActivations}_{trace}$ is empty).
\begin{algorithm2e}[t!]
\tiny
\DontPrintSemicolon \SetAlgoVlined
\KwIn{$log$, the event log to be processed; $(a,t)$, activation and target of a reference constraint; $\varphi_a$, $\varphi_c$, and $\varphi_t$ activation, correlation, and time condition of the reference constraint}
\BlankLine
define vectors $\textit{fulfillments}$ and $\textit{violations}$, containing the fulfillments and the violations in each trace with respect to the given constraint.
\ForEach{$trace \in log$} {
define vectors $\textit{fulfillments}_{trace}$ and $\textit{violations}_{trace}$, containing the fulfillments and the violations in trace $trace$ with respect to the reference constraint \;
    define vector $\textit{pendingActivations}_{trace}$ containing events corresponding to pending activations in trace $trace$ \;
   \ForEach{$event \in trace$} {\label{line:loop}
       \If{$event.name = a ~\&\&~ check_a(\varphi_a,event)$} {
            $\textit{pendingActivations}_{trace}.\text{add}(event)$ \;
        }
        \If{$event.name = t$} {
            \ForEach{$p \in \textit{pendingActivations}_{trace}$} {
                \If{$check_c(\varphi_c,p,event) ~\&\&~ check_t(\varphi_t,p,event)$} {
                      $\textit{pendingActivations}_{trace}.\text{remove}(p)$ \;
                     $\textit{fulfillments}.\text{add}(p)$ \;
                }
            }
        }
    }
    \ForEach{$p \in \textit{pendingActivations}_{trace}$} {
    $\textit{pendingActivations}_{trace}.\text{remove}(p)$ \;
    $\textit{violations}.\text{add}(p)$ \;
    }
    $\textit{fulfillments}.\text{add}(\textit{fulfillments}_{trace})$ \;
$\textit{violations}.\text{add}(\textit{violations}_{trace})$ \;
}
\BlankLine
\KwOut{$\textit{fulfillments}$ and $\textit{violations}$, two list of vectors (one per trace) containing the fulfillments and the violations in each trace with respect to the given constraint.}
\caption{Conformance checking algorithm for response. \label{alg:response}}
\end{algorithm2e}





The algorithm for the conformance checking of a log with respect to \emph{precedence} constraints is similar to the one described for response. The difference is that, for precedence constraints, we iterate each trace in the event log (line 4) from the last event to the first one. In the algorithm for the conformance checking of a log with respect to \emph{responded existence} constraints, we iterate each trace in the log in both directions. If for an activation there is a corresponding target following it in one of the two directions, the activation is a fulfillment otherwise it is a violation.

%The algorithm receives as input an event $e = (c, a, t)$, where $c$ is the case
%id, $a$ is the activity name and $t$ is the timestamp. This event is processed
%by updating maps \textit{activationsCounter}$_c$ and
%\textit{pendingActivations}$_c$. If $c$ is a new case, these maps are first
%defined (lines \ref{alg:response:map1}-\ref{alg:response:map2}).

%Then, if $a$ has never occurred in $c$ (i.e., if $a$ is not in
%\textit{activationsCounter}$_c$), $a$ is added as a key in
%\textit{activationsCounter}$_c$ with number of occurrences equal to 1 ($a$ has
%occurred only once in $c$).
%Lines \ref{alg:response:sins}-\ref{alg:response:sins2} of the algorithm are used
%to update map \textit{pendingActivations}$_c$ when $a$ occurs in $c$ for the first time. In
%particular, all the response constraints having $a$ as second parameter cannot
%have any pending activation when $a$ occurs (all of them are fulfilled when $a$ occurs).
%Therefore, line \ref{alg:response:sins1} of the algorithm sets to 0 the number of pending
%activations in $c$ for the response constraints having $a$ as second parameter.
%On the other hand, all the response constraints having $a$ as first parameter
%are activated when $a$ occurs and waiting for some other event to occur. Then,
%$a$ is a pending activation for these constraints (and the only one).
%Therefore, line \ref{alg:response:sins2} of the algorithm sets to 1 the number of pending
%activations in $c$ for the response constraints having $a$ as first parameter.

%If $a$ has already occurred in $c$ (i.e., if $a$ is already in
%\textit{activationsCounter}$_c$), the number of occurrences of $a$ is
%incremented by 1 in \textit{activationsCounter}$_c$.
%Line \ref{alg:response:pend0} of the algorithm sets to 0 the pending activations
%in $c$ for the response constraints having $a$ as second parameter. On the other
%hand, all the response constraints having $a$ as first parameter are activated
%when $a$ occurs and, therefore, the number of pending activations for these
%constraints in $c$ is incremented by 1.
%Finally (line \ref{alg:response:adds}), if activity name $a$ is observed for the
%first time in the event stream, $a$ is added to $L$.

%Using the algorithm just described it is possible to count the number of
%activations for every candidate response constraint (using maps
%\textit{activationsCounter}$_c$), and the number of violations (counting the
%number of activations still pending in maps \textit{pendingActivations}$_c$).
%These metrics are enough for deriving, at any point in time, \emph{fulfillment
%ratio} and \emph{violation ratio} for (not) response constraints.



\subsection{Multi-Perspective Alternate Response and Alternate Precedence}
\label{response}

The algorithm presented in this section (Algorithm~\ref{alg:alternate}) can be used for the discovery of
\emph{alternate response} constraints.
%We illustrate the algorithm (Algorithm~\ref{alg:response})
%for the response template. The algorithm is identical for the not response
%template, since the fulfillment ratio for a response constraint corresponds to
%the violation ratio of the not response constraint over the same activities (and
%vice versa).\footnote{A similar observation also applies to the algorithms described in the following sections.}
In the same way as illustrated for response and precedence constraints, also in this case a similar algorithm is able to discover
\emph{alternate precedence} constraints.


\begin{algorithm2e}[t!]
\tiny
\DontPrintSemicolon \SetAlgoVlined
\KwIn{$log$, the event log to be processed; $(a,t)$, activation and target of a reference constraint; $\varphi_a$, $\varphi_c$, and $\varphi_t$ activation, correlation, and time condition of the reference constraint}
\BlankLine
define vectors $\textit{fulfillments}$ and $\textit{violations}$, containing the fulfillments and the violations in each trace with respect to the given constraint.
\ForEach{$trace \in log$} {
define vectors $\textit{fulfillments}_{trace}$ and $\textit{violations}_{trace}$, containing the fulfillments and the violations in trace $trace$ with respect to the reference constraint \;
    define vector $\textit{pendingActivations}_{trace}$ containing events corresponding to pending activations in trace $trace$ \;
    define vector $\textit{possibleTargets}_{trace}$ containing possible target events corresponding to a pending activation \;
    \ForEach{$event \in trace$} {
        \If{$event.name = a ~\&\&~ check_a(\varphi_a,event)$} {
            \If{$\textit{possibleTargets}_{trace}.\text{size} \geqslant 1 ~ \&\& ~ \textit{pendingActivations}_{trace}.\text{size} = 1$}{
                $targetFound := false$ \;
                $previousAct := element \in \textit{pendingActivations}_{trace}$ \;
                \ForEach{$p \in \textit{possibleTargets}_{trace}$} {
                  \If{$check_c(\varphi_c,previousAct,p) ~\&\&~ check_t(\varphi_t,previousAct,p)$} {
                        $targetFound := true$\;
                        $\textit{pendingActivations}_{trace}.\text{remove}(previousAct)$ \;
                      $\textit{fulfillments}.\text{add}(previousAct)$ \;
                    }
                }
                \If{$!targetFound$}{
                     $\textit{pendingActivations}_{trace}.\text{remove}(previousAct)$ \;
                      $\textit{violations}.\text{add}(previousAct)$ \;
                }
            }
            \If{$\textit{possibleTargets}_{trace}.\text{size} = 0 ~ \&\& ~ \textit{pendingActivations}_{trace}.\text{size} = 1$}{
                  $previousAct := element \in \textit{pendingActivations}_{trace}$ \;
                    $\textit{pendingActivations}_{trace}.\text{remove}(previousAct)$ \;
                      $\textit{violations}.\text{add}(previousAct)$ \;
            }
            $\textit{possibleTargets}_{trace}.\text{removeAll()}$ \;
            $\textit{pendingActivations}_{trace}.\text{add}(event)$ \;
        }
        \If{$event.name = t$} {
           $\textit{possibleTargets}_{trace}.\text{add}(event)$ \;
        }
    }
    \If{$\textit{possibleTargets}_{trace}.\text{size} \geqslant 1 ~ \&\& ~ \textit{pendingActivations}_{trace}.\text{size} = 1$}{
        $targetFound := false$ \;
        $previousAct := element \in \textit{pendingActivations}_{trace}$ \;
        \ForEach{$p \in \textit{possibleTargets}_{trace}$} {
              \If{$check_c(\varphi_c,previousAct,p) ~\&\&~ check_t(\varphi_t,previousAct,p)$} {
                        $targetFound := true$\;
                        $\textit{pendingActivations}_{trace}.\text{remove}(previousAct)$ \;
                      $\textit{fulfillments}.\text{add}(previousAct)$ \;
                    }
                }
                \If{$!targetFound$}{
                     $\textit{pendingActivations}_{trace}.\text{remove}(previousAct)$ \;
                      $\textit{violations}.\text{add}(previousAct)$ \;
                }
 }
 $\textit{fulfillments}.\text{add}(\textit{fulfillments}_{trace})$ \;
$\textit{violations}.\text{add}(\textit{violations}_{trace})$ \;
}
\BlankLine
\KwOut{$\textit{fulfillments}$ and $\textit{violations}$, two list of vectors (one per trace) containing the fulfillments and the violations in each trace with respect to the given constraint.}
\caption{Discovery algorithm for alternate response. \label{alg:alternate}}
\end{algorithm2e}


The inputs of this algorithm are an event log $log$, a multi-perspective constraint with activation $a$, target $t$, activation condition $\varphi_a$, correlation condition $\varphi_a$, and time condition $\varphi_t$. The outputs of the algorithm are two lists of vectors $\textit{fulfillments}$ and $\textit{violations}$ (one of each per trace) containing the fulfillments and the violations in each trace with respect to the given constraint.


For each trace $trace$ in $log$, vectors $\textit{fulfillments}_{trace}$ and $\textit{violations}_{trace}$ contain the fulfillments and the violations in trace $trace$ with respect to the reference constraint. $\textit{pendingActivations}_{trace}$ is a vector containing the pending activations in $trace$ for the input
constraint. $\textit{possibleTargets}_{trace}$ is a vector containing the possible targets for the last pending activation encountered in $trace$ and added to $\textit{pendingActivations}_{trace}$.

For each event $event$ in $trace$, if the event name of $event$ is equal to $a$ and condition $\varphi_a$ is satisfied on the payload of $event$, the constraint is activated in $trace$ (line 6). In this case, the algorithm checks if there is one pending activation ($previousAct$) in $\textit{pendingActivations}_{trace}$ and there is at least one possible corresponding target in $\textit{possibleTargets}_{trace}$ for this activation (line 7). If this is the case, the algorithm checks if $previousAct$ can be correlated to one of the possible targets in $\textit{possibleTargets}_{trace}$ (through functions $check_c$ and $check_t$). If $previousAct$ has a correlated target, then $previousAct$ is removed from $\textit{pendingActivations}_{trace}$ and added to $\textit{fulfillments}_{trace}$ (lines 13 and 14), otherwise it is moved to $\textit{violations}_{trace}$ (lines 16 and 17), since an alternate response constraint does not allow two activations to occur one after another without any target in between (see Table\ref{}). For the same reason, $previousAct$ is moved to $\textit{violations}_{trace}$ if $\textit{possibleTargets}_{trace}$ is empty (lines 20 and 21). In all cases, when $event$ is an activation, all elements in $\textit{possibleTargets}_{trace}$ are deleted and $event$ is added to $\textit{pendingActivations}_{trace}$ (lines 22 and 23). If $event$ is a target of the reference constraint, $event$ is added to $\textit{possibleTargets}_{trace}$ (line 25).
After that the last event in $trace$ has been processed, the algorithm checks again if there is still one pending activation in $\textit{pendingActivations}_{trace}$ with at least one possible corresponding target in $\textit{possibleTargets}_{trace}$. If this is the case, the algorithm checks if the pending activation can be correlated to one of the possible targets. If there is a correlated target, the activation is moved to $\textit{fulfillments}_{trace}$ (lines 32 and 33), otherwise it is moved to $\textit{violations}_{trace}$ (lines 35 and 36).

%If $event$ is an activation, there is already one pending activation ($previousAct$) in $\textit{pendingActivations}_{trace}$ and there are no possible corresponding targets for this activation ($\textit{possibleTargets}_{trace}$ is empty), then $previousAct$ is added to $\textit{violations}_{trace}$ (line 21) since an alternate response constraint does not allow two activations to occur one after another without any target in between (see Table 1).

%Finally, if $event$ is an activation and $event$ is preceded by at least one possible target, then all the elements in $\textit{pendingActivations}_{trace}$ are deleted (line 23). In all cases, when $event$ is an activation, all elements in $\textit{possibleTargets}_{trace}$ are deleted and $event$ is added to $\textit{pendingActivations}_{trace}$ (lines 24 and 25). If $event$ is a target of the candidate constraint under examination, $event$ is added to $\textit{possibleTargets}_{trace}$ (line 27).

%The candidate constraint is non-vacuously satisfied in $trace$, if, when all the events in $trace$ have been processed, the boolean variable $activated$ is true ($trace$ contains at least one activation of the candidate constraint), $\textit{pendingActivations}_{trace}$ is empty and the boolean variable $violated$ is false.


\begin{algorithm2e}[t!]
\tiny
\DontPrintSemicolon \SetAlgoVlined
\KwIn{$log$, the event log to be processed; $(a,t)$, activation and target of a reference constraint; $\varphi_a$, $\varphi_c$, and $\varphi_t$ activation, correlation, and time condition of the reference constraint}
\BlankLine
define vectors $\textit{fulfillments}$ and $\textit{violations}$, containing the fulfillments and the violations in each trace with respect to the given constraint.
\ForEach{$trace \in log$} {
define vectors $\textit{fulfillments}_{trace}$ and $\textit{violations}_{trace}$, containing the fulfillments and the violations in trace $trace$ with respect to the reference constraint \;
    define vector $\textit{pendingActivations}_{trace}$ containing events corresponding to pending activations in trace $trace$ \;
    \ForEach{$event \in trace$} {
        \If{$\textit{pendingActivations}_{trace}.\text{size} = 1$}{
            $p := element \in \textit{pendingActivations}_{trace}$ \;
            \eIf{$event.name = t$} {
                \eIf{$check_c(\varphi_c,p,event) ~\&\&~ check_t(\varphi_t,p,event)$} {
                      $\textit{pendingActivations}_{trace}.\text{remove}(p)$ \;
                      $\textit{fulfillments}.\text{add}(p)$ \;
                }{
                     $\textit{pendingActivations}_{trace}.\text{remove}(p)$ \;
                      $\textit{violations}.\text{add}(p)$ \;
                }
            } {
                $\textit{pendingActivations}_{trace}.\text{remove}(p)$ \;
                      $\textit{violations}.\text{add}(p)$ \;
            }
           % $\textit{pendingActivations}_{trace}.\text{removeAll()}$ \;
        }
        \If{$event.name = a ~\&\&~ check_a(\varphi_a,event)$} {
            $\textit{pendingActivations}_{trace}.\text{add}(event)$ \;
        }
    }
$\textit{fulfillments}.\text{add}(\textit{fulfillments}_{trace})$ \;
$\textit{violations}.\text{add}(\textit{violations}_{trace})$ \;
}
\BlankLine
\KwOut{$\textit{fulfillments}$ and $\textit{violations}$, two list of vectors (one per trace) containing the fulfillments and the violations in each trace with respect to the given constraint.}
\caption{Discovery algorithm for chain response. \label{alg:chain}}
\end{algorithm2e}

\subsection{Multi-Perspective Chain Response and Chain Precedence}
\label{response}

The algorithm presented in this section (Algorithm~\ref{alg:chain}) can be used for the discovery of
\emph{chain response} constraints.
A similar algorithm is able to discover
\emph{chain precedence} constraints.


The inputs of this algorithm are an event log $log$, a multi-perspective constraint with activation $a$, target $t$, activation condition $\varphi_a$, correlation condition $\varphi_a$, and time condition $\varphi_t$. The outputs of the algorithm are two lists of vectors $\textit{fulfillments}$ and $\textit{violations}$ (one of each per trace) containing the fulfillments and the violations in each trace with respect to the given constraint.

For each trace $trace$ in $log$, vectors $\textit{fulfillments}_{trace}$ and $\textit{violations}_{trace}$ contain the fulfillments and the violations in trace $trace$ with respect to the reference constraint. $\textit{pendingActivations}_{trace}$ is a vector containing the pending activations in $trace$ for the reference constraint under examination.


For each event $event$ in $trace$, if $event$ is an activation (the event name of $event$ is equal to $a$ and condition $\varphi_a$ is satisfied on the payload of $event$), it is added to $\textit{pendingActivations}_{trace}$ (lines 17 and 18). If $\textit{pendingActivations}_{trace}$ contains an element, and $event$ is a target event, then the algorithm checks if the pending activation in $\textit{pendingActivations}_{trace}$ can be correlated to $event$ (the algorithm checks if this is the case through functions $check_c$ and $check_t$). If the two events can be correlated, the activation is moved to $\textit{fulfillments}_{trace}$ (line 10), otherwise it is moved to $\textit{violations}_{trace}$ (line 13). A violation is detected also if $\textit{pendingActivations}_{trace}$  contains an activation and the current event $event$ is not a target event (lines 15 and 16), since,
%the algorithm guarantees that if $\textit{pendingActivations}_{trace}$  contains an activation, the current processed event $event$ must be the event that immediately follows the activation in $\textit{pendingActivations}_{trace}$. This is always the case since if the algorithm processes an event and there is an activation in $\textit{pendingActivations}_{trace}$, this activation is anyway removed from this vector (line 17). Therefore, if $\textit{pendingActivations}_{trace}$  contains an activation and the current processed event $event$ is not a target,
according to the semantics of the chain response, a target should immediately follow an activation.
After that the last event in $trace$ has been processed, the algorithm checks if there is still one pending activation in $\textit{pendingActivations}_{trace}$. If this is the case, the activation is moved to $\textit{violations}_{trace}$.





%\begin{algorithm2e}[t]
%\tiny
%\DontPrintSemicolon \SetAlgoVlined
%\KwIn{$log$, the event log to be processed; $(a,t)$, activation and target of a candidate constraint; $corr$ a selected correlation for linking each activation with the corresponding target}
%\BlankLine
%define vector $\textit{timeDistances}$ containing the time distances between each activation and the corresponding targets \;
%\BlankLine
%\ForEach{$trace \in log$} {
 %   define vector $\textit{pendingActivations}_{trace}$ containing events corresponding to pending activations in trace $trace$ \;
 %   \ForEach{$event \in trace$} {\label{line:loop}
 %       \If{$event.name = a$} {
 %           $\textit{pendingActivations}_{trace}.\text{add}(event)$ \;
 %       }
 %       \If{$event.name = t$} {
 %           \ForEach{$p \in \textit{pendingActivations}_{trace}$} {
  %              \If{$\textit{isValid}(corr,p,event)$} {
   %                   $\textit{pendingActivations}_{trace}.\text{remove}(p)$ \;
   %                   $\textit{timeDistances}.\text{add}(|p.timestamp - event.timestamp|)$ \;
    %            }
    %        }
    %    }
   % }
%}
%\BlankLine
%\KwOut{$\textit{timeDistances}$}
%\caption{Discovery algorithm for timed not response. \label{alg:notresponse}}
%\end{algorithm2e}


%\subsection{Timed Not Response, Not Precedence, and Not Responded Existence}
%\label{response}

%The algorithm presented in this section can be used for the discovery of
%\emph{timed not response} constraints. As discussed for timed response, precedence, and responded existence, with a similar algorithm it is possible to discover also
%\emph{timed not precedence} and \emph{timed not responded existence} constraints.


%The inputs of this algorithm are an event log $log$, a candidate constraint with activation $a$ and target $t$ and a feasible correlation $corr$. The outputs of the algorithm are the vector $\textit{timeDistances}$ containing the time distances between each activation of the candidate constraint and the corresponding targets, and the support of the candidate constraint $support$, i.e., the ratio between the number of traces in which the constraint is satisfied ($validTracesNumber$) and the total number of traces in the event log.

%For each trace $trace$ in $log$, $\textit{pendingActivations}_{trace}$ is a vector containing the pending activations in $trace$ for the candidate
%constraint under examination, i.e., the activations that do not have a corresponding target. For event $event$ in $trace$, if $event$ is an activation for the candidate constraint, $event$ is added to $\textit{pendingActivations}_{trace}$. If $event$ is a target for the candidate constraint, then for each pending activation $p$ in $\textit{pendingActivations}_{trace}$, if $p$ can be correlated to $event$ through correlation $corr$ (the algorithm checks if this is the case through function $isValid$), then $p$ is removed from the set of pending activation and the time distance between $p$ and the corresponding target $event$ is added to $\textit{timeDistances}$. The candidate constraint under examination is non vacuously satisfied in trace $trace$, if an activation is occurred at least once.





%The algorithm for the discovery of \emph{timed precedence} constraints is similar to the one described for timed response. The difference is that, for timed precedence constraints, we iterate each trace in the event log (line 5) from the last event to the first one. In the algorithm for the discovery of \emph{timed responded existence} constraints, we iterate each trace in the log in both directions so that each activation can have zero, one, or two possible targets. If there are no possible target, there is a violation in the trace. If there is only one possible target we evaluate the time distance between the activation and the corresponding target. If there are two possible targets, we consider the one with the smallest time distance from the considered activation.

%\subsection{Time Intervals Identification}
%\label{sec:interval}
%In this section, we describe how the time distances generated by the discovery algorithm described so far can be used to
%derive statistics on the delays between activations and targets of the candidate constraint. In particular, they are used to
%identify the time interval $[t_1,t_2]$ characterizing the discovered metric temporal constraint. Suppose that $d_{min}$ and $d_{max}$ are the %minimum and the maximum time distances between an activation and the corresponding target of the candidate constraint under examination. Then, if the candidate constraint is a positive relation constraint, we simply derive that $t_1 = d_{min}$ and $t_2 = d_{max}$.


%Also in the case of a negative relation constraint, if an activation occurs at time $t$ all the possible targets for that activations occur at a time point belonging to the interval $[t+d_{min},t+d_{max}]$. However, in case of a negative relation constraint, the constraint is valid outside this interval.
 %$[d_{min},d_{max}]$.
% Therefore, we can associate two intervals to the candidate constraint (thus discovering two constraints from it), i.e., $[0,d_{min}[$ and $]d_{max},\infty[$.

% To deal with cases in which logs contain noise, it is also possible to choose the boundaries of the time intervals by removing outliers from the discovered set of time distances. This can easily be done by removing time distances that deviate more than a given threshold from the average.


